CAT-ORA: Collision-Aware Time-Optimal Formation Reshaping for Efficient Robot Coordination in 3D Environments

In this paper, we introduce an algorithm designed to address the problem of time-optimal formation reshaping in three-dimensional environments while preventing collisions between agents. The utility of the proposed approach is particularly evident in mobile robotics, where agents benefit from being organized and navigated in formation for a variety of real-world applications requiring frequent alterations in formation shape for efficient navigation or task completion. Given the constrained operational time inherent to battery-powered mobile robots, the time needed to complete the formation reshaping process is crucial for their efficient operation, especially in case of multi-rotor Unmanned Aerial Vehicles (UAVs). The proposed Collision-Aware Time-Optimal formation Reshaping Algorithm (CAT-ORA) builds upon the Hungarian algorithm for the solution of the robot-to-goal assignment implementing the inter-agent collision avoidance through direct constraints on mutually exclusive robot-goal pairs combined with a trajectory generation approach minimizing the duration of the reshaping process. Theoretical validations confirm the optimality of CAT-ORA, with its efficacy further showcased through simulations, and a real-world outdoor experiment involving 19 UAVs. Thorough numerical analysis shows the potential of CAT-ORA to decrease the time required to perform complex formation reshaping tasks by up to 49%, and 12% on average compared to commonly used methods in randomly generated scenarios.

==> fig/trapezoids/lsap_vs_blap_ratio_illustration.tex <==
\begin{tikzpicture}[line cap=round]
  \coordinate (zero) at (0,0);
  \coordinate (s1) at (-180:3.0);
  \coordinate (s2) at (160:3.0);
  \coordinate (s3) at (120:3.0);
  \coordinate (s4) at (80:3.0);
  \coordinate (s5) at (40:3.0);
  \coordinate (g1) at (0:3.0);
  \coordinate (g2) at (150:3.0);
  \coordinate (g3) at (110:3.0);
  \coordinate (g4) at (70:3.0);
  \coordinate (g5) at (30:3.0);
  % \coordinate (sj) at ( 80:1.4);
  % \coordinate (gi) at ( 25:3.3);
  % \coordinate (A+B) at ($(A)+(B)$);

  % \draw[ultra thick, dashed, mypurple!40] (sj) -- (gj) node[midway,above] {$Md$};
  % \draw[ultra thick, dashed, mypurple!40] (si) -- (gj) node[midway,below] {$d$};

  \draw[myblue,fill=myblue] (s1) circle (.5ex) node[midway,above, shift={(-3.3, 0.0)}] {$\mathbf{s}_1$};
  \draw[myblue,fill=myblue] (s2) circle (.5ex) node[midway,above, shift={(-3.1, 0.7)}] {$\mathbf{s}_2$};
  \draw[myblue,fill=myblue] (s3) circle (.5ex) node[midway,above, shift={(-1.8, 2.4)}] {$\mathbf{s}_3$};
  \draw[myblue,fill=myblue] (s4) circle (.5ex) node[midway,above, shift={(0.2, 2.8)}] {$\mathbf{s}_4$};
  \draw[myblue,fill=myblue] (s5) circle (.5ex) node[midway,above, shift={(2.2, 2.0)}] {$\mathbf{s}_5$};
  \draw[myred,fill=myred] (g1) circle (.5ex) node[midway,below, shift={(-2.8, 2.0)}] {$\mathbf{g}_1$};
  \draw[myred,fill=myred] (g2) circle (.5ex) node[midway,below, shift={(-0.8, 3.3)}] {$\mathbf{g}_2$};
  \draw[myred,fill=myred] (g3) circle (.5ex) node[midway,below, shift={(1.4, 3.1)}] {$\mathbf{g}_3$};
  \draw[myred,fill=myred] (g4) circle (.5ex) node[midway,below, shift={(2.9, 1.6)}] {$\mathbf{g}_4$};
  \draw[myred,fill=myred] (g5) circle (.5ex) node[midway,below, shift={(3.4, 0.3)}] {$\mathbf{g}_5$};
  
  \draw[vector,arrow,myred,opacity=0.8] (s1) -- (g2) node[midway,right] {$\mathbf{p}_{1,1}$};
  \draw[vector,arrow,myred,opacity=0.8] (s2) -- (g3) node[midway,below right] {$\mathbf{p}_{2,2}$};
  \draw[vector,arrow,myred,opacity=0.8] (s3) -- (g4) node[midway,below] {$\mathbf{p}_{3,3}$};
  \draw[vector,arrow,myred,opacity=0.8] (s4) -- (g5) node[midway,below] {$\mathbf{p}_{4,4}$};
  \draw[vector,arrow,myred,opacity=0.8] (s5) -- (g1) node[midway,left] {$\mathbf{p}_{5,5}$};

  \draw[vector,arrow,myblue,opacity=0.8] (s1) -- (g1) node[midway,above] {$\mathbf{p}_{1,5}$};
  \draw[vector,arrow,myblue,opacity=0.8] (s2) -- (g2) node[midway, left, shift={(0.0, 0.1)}] {$\mathbf{p}_{2,1}$};
  \draw[vector,arrow,myblue,opacity=0.8] (s3) -- (g3) node[midway,above, shift={(-0.15, 0.0)}] {$\mathbf{p}_{3,2}$};
  \draw[vector,arrow,myblue,opacity=0.8] (s4) -- (g4) node[midway,above] {$\mathbf{p}_{4,3}$};
  \draw[vector,arrow,myblue,opacity=0.8] (s5) -- (g5) node[midway, right, shift={(0.0, 0.1)}] {$\mathbf{p}_{5,4}$};

  % \draw[vector,arrow,myred] (gj) -- (gi) node[midway,above right] {$\mathbf{G}_{ji}$};
  % \draw[vector,arrow,mypurple] (O) -- (A+B) node[above right=-3] {$\vb{a}+\vb{b}$};

  % \draw[vector,thin arrow,myblue!40] (A) -- (A+B) node[midway,below right=-2] {$\vb{b}$};
\end{tikzpicture}

